RELATIO: Text Semantics Capture Political and Economic Narratives

Social scientists have become increasingly interested in how narratives -- the stories in fiction, politics, and life -- shape beliefs, behavior, and government policies. This paper provides an unsupervised method to quantify latent narrative structures in text documents. Our new software package RELATIO identifies coherent entity groups and maps explicit relations between them in the text. We provide an application to the United States Congressional Record to analyze political and economic narratives in recent decades. Our analysis highlights the dynamics, sentiment, polarization, and interconnectedness of narratives in political discourse.

==> stopwords.tex <==
\footnotesize

i
me
my
myself    
we 
us
our            
ours           
ourselves      
you            
your          
yours         
yourself       
yourselves    
he             
him           
his           
himself      
she            
her            
hers           
herself       
it             
its            
itself         
they           
them           
their          
theirs         
themselves     
what
which
who
whom
this
that
these
those
a
an
the
and
but
if
or
because
as
until
while
of
at
by
for
with
about
against
between
into
through
during
before
after
above
below
to
from
up
down
in
out
on
off
over
under
again
further
then
once
here
there
when
where
why
how
all
any
both
each
few
more
most
other
some
such
no
nor
not
only
own
same
so
than
too
very
much
actual
abraham
aderholt
adler
akaka
alexander
allard
allen
amash
amodei
andrews
applegate
archer
arcuri
armey
ashcroft
ayotte
bacchus
bachmann
bachus
baesler
baird
baker
baldacci
baldwin
ballance
ballenger
barber
barca
barcia
barkley
barletta
barlow
barr
barrasso
barrett
barrow
barton
bass
bateman
baucus
bayh
bean
beatty
beauprez
becerra
begich
beilenson
bell
benishek
bennet
bennett
bentivolio
bentley
bentsen
bera
bereuter
berry
bevill
biden
bilbray
bilirakis
bingaman
bishop
black
blackburn
blackwell
blagojevich
bliley
blumenauer
blumenthal
blunt
blute
boccieri
boehlert
boehner
bonamici
bond
bonilla
bonior
bono
boozman
boren
borski
boucher
boustany
boxer
boyd
boyda
bradley
brady
braley
breaux
brewster
bridenstine
bright
brooks
broun
browder
brown
brownback
brownley
bryan
bryant
buchanan
bucshon
bumpers
bunn
bunning
burgess
burns
burr
burris
bustos
butterfield
buyer
byrd
byrne
callahan
calvert
camp
campbell
canady
cannon
cantor
cantwell
cao
capito
capps
capuano
cardenas
cardin
carnahan
carney
carper
carson
carter
cartwright
case
casey
cassidy
castle
castor
castro
cazayoux
chabot
chafee
chaffetz
chambliss
chapman
chiesa
childers
chocola
christensen
chrysler
chu
cicilline
clarke
clay
clayton
cleaver
cleland
clement
clinger
clinton
clyburn
coats
coble
coburn
cochran
coffman
cohen
cole
coleman
collins
combest
conaway
condit
connolly
conrad
conyers
cook
cooksey
cooley
coons
cooper
coppersmith
corker
cornyn
corzine
costa
cotton
courtney
coverdell
cox
coyne
craig
cramer
crane
crapo
crawford
cremeans
crenshaw
crowley
cruz
cubin
cuellar
culberson
cummings
cunningham
dahlkemper
daines
danforth
danner
darden
daschle
davis
dayton
deal
deconcini
defazio
degette
delahunt
delaney
delauro
delay
dellums
denham
dent
derrick
deutch
deutsch
dewine
dickey
dingell
dixon
djou
dodd
doggett
dole
domenici
donnelly
dooley
doolittle
dorgan
doyle
drake
driehaus
duckworth
duffy
duncan
dunn
durbin
durenberger
edwards
ehlers
ehrlich
ellison
ellmers
ellsworth
emanuel
emerson
engel
english
ensign
enyart
enzi
eshoo
esty
etheridge
evans
everett
ewing
exon
faircloth
fallin
farenthold
farr
fattah
fawell
fazio
feeney
feingold
feinstein
ferguson
fields
fincher
fingerhut
fischer
fish
fitzgerald
fitzpatrick
flake
flanagan
fleischmann
fleming
fletcher
flores
foley
forbes
ford
fortenberry
fossella
foster
fowler
fox
foxx
frahm
frankel
franken
franks
frelinghuysen
frisa
frist
frost
fudge
funderburk
furse
gabbard
gallego
gallo
ganske
garamendi
garcia
gardner
garrett
gejdenson
gekas
gephardt
geren
gerlach
gibbons
gibbs
gibson
giffords
gilchrest
gillibrand
gillmor
gilman
gingrey
gingrich
glenn
glickman
gohmert
gonzalez
goode
goodlatte
goodling
goodwin
gordon
gorton
gosar
goss
gowdy
graham
gramm
grams
grandy
granger
grassley
graves
grayson
green
greene
greenwood
gregg
griffin
griffith
grijalva
grimm
grucci
gunderson
guthrie
gutierrez
gutknecht
hagan
hagel
hahn
hall
halvorson
hamburg
hamilton
hanabusa
hancock
hanna
hansen
hare
harkin
harman
harper
harris
hart
hartzler
hastert
hastings
hatch
hatfield
hayes
hayworth
heck
hefley
heflin
hefner
heineman
heinrich
heitkamp
heller
helms
hensarling
herrera
higgins
hill
hilleary
hilliard
himes
hinojosa
hirono
hoagland
hobson
hochbrueckner
hodes
hoeffel
hoekstra
hoeven
hoke
holding
hollings
holt
honda
hooley
horn
horsford
hostettler
houghton
hoyer
hudson
huelskamp
huffington
huffman
hughes
huizenga
hulshof
hultgren
hunter
hurt
hutchinson
hutchison
hutto
hyde
inglis
inhofe
inouye
inslee
isakson
israel
issa
istook
jackson
janklow
jefferson
jeffords
jeffries
jenkins
jindal
johanns
john
johnson
johnston
jones
jordan
joyce
kagen
kaine
kanjorski
kaptur
kasich
kassebaum
kaufman
keating
keller
kelly
kempthorne
kennedy
kennelly
kerns
kerrey
kerry
kildee
kilmer
kilpatrick
kilroy
kim
kind
king
kingston
kinzinger
kirk
kirkpatrick
kleczka
klein
kline
klink
klobuchar
klug
knollenberg
kohl
kolbe
kopetski
kosmas
kratovil
kreidler
kuhl
kuster
kuykendall
kyl
labrador
lafalce
lamborn
lampson
lancaster
lance
landrieu
langevin
lankford
lantos
largent
larsen
larson
latham
latta
laughlin
lautenberg
lazio
leach
leahy
lee
lehman
levin
levy
lewis
lieberman
lightfoot
lincoln
linder
lipinski
livingston
lloyd
lobiondo
loebsack
lofgren
long
longley
lott
lowenthal
lowey
lucas
luetkemeyer
lugar
lujan
lummis
luther
lynch
machtley
mack
maffei
mahoney
majette
maloney
manchin
mann
manton
marchant
marino
markey
marshall
martinez
martini
mascara
massa
massie
matheson
mathews
matsui
mazzoli
mccain
mccandless
mccarthy
mccaskill
mccaul
mcclintock
mccloskey
mccollum
mcconnell
mccrery
mccurdy
mcdermott
mcgovern
mchale
mchenry
mchugh
mcinnis
mcintosh
mcintyre
mckeon
mckinley
mckinney
mcleod
mcmahon
mcmillan
mcnerney
mcnulty
meadows
meehan
meek
meeks
melancon
menendez
meng
merkley
messer
metcalf
meyers
mfume
mica
michaud
michel
mikulski
miller
mineta
minge
minnick
mitchell
moakley
molinari
mollohan
montgomery
moore
moorhead
moran
morella
moynihan
mullin
mulvaney
murkowski
murphy
murray
murtha
musgrave
myers
nadler
napolitano
natcher
neal
nelson
nethercutt
neugebauer
neumann
ney
nickles
noem
nolan
northup
norwood
nugent
nunes
nunn
nunnelee
nussle
nye
obama
oberstar
obey
olson
ortiz
orton
osborne
ose
otter
owens
oxley
packard
packwood
palazzo
pallone
pappas
parker
pascrell
pastor
paul
paulsen
paxon
payne
pearce
pease
pell
pelosi
penny
perlmutter
perriello
perry
peters
peterson
petri
phelps
pickering
pickett
pickle
pingree
pittenger
pitts
pocan
poe
polis
pombo
pomeroy
pompeo
porter
portman
posey
poshard
pressler
price
pryce
pryor
putnam
quigley
quillen
quinn
radanovich
radel
rahall
ramstad
rangel
ravenel
redmond
reed
regula
reichert
reid
renacci
renzi
reynolds
ribble
rice
richardson
richmond
ridge
riegle
rigell
riley
risch
rivers
robb
roberts
roby
rockefeller
rodgers
rodriguez
roe
roemer
rogan
rogers
rohrabacher
rokita
rooney
ros
rose
roskam
ross
rostenkowski
roth
rothfus
roukema
rowland
royce
rubio
ruiz
runyan
ruppersberger
rush
ryan
ryun
sabo
salazar
sali
salmon
sanchez
sanders
sandlin
sanford
sangmeister
santorum
sarbanes
sarpalius
sasser
sawyer
saxton
scalise
scarborough
schaefer
schaffer
schakowsky
schatz
schauer
schenk
schiff
schneider
schock
schrader
schrock
schroeder
schultz
schumer
schwartz
schwarz
schweikert
scott
seastrand
sekula
sensenbrenner
serrano
sessions
sestak
sewell
shadegg
shaheen
sharp
shaw
shays
shelby
shepherd
sherman
sherwood
shimkus
shows
shuster
simmons
simon
simpson
sinema
sires
sisisky
skaggs
skeen
slattery
slaughter
smith
snowbarger
snowe
snyder
sodrel
solis
souder
southerland
space
specter
speier
spence
spratt
stabenow
stenholm
stevens
stewart
stivers
stockman
stokes
strickland
studds
stupak
stutzman
sundquist
sununu
swalwell
sweeney
swett
swift
synar
takano
talent
tancredo
tanner
tate
tauscher
tauzin
taylor
tejeda
terry
tester
thomas
thompson
thornberry
thune
thurman
thurmond
tiahrt
tiberi
tierney
tipton
titus
tonko
toomey
torkildsen
torres
torricelli
traficant
tsongas
tucker
turner
udall
unsoeld
upton
valadao
valentine
van
vargas
veasey
vela
velazquez
vento
visclosky
vitter
voinovich
volkmer
vucanovich
wagner
walberg
walden
walker
wallop
walorski
walsh
walz
wamp
ward
warner
warren
waters
watson
watt
watts
waxman
webb
weber
webster
weiner
welch
weldon
weller
wellstone
wenstrup
westmoreland
wexler
weygand
wheat
white
whitehouse
whitfield
whitten
wicker
williams
wilson
wise
wittman
wofford
wolf
womack
woodall
wu
wyden
wynn
yarmuth
yoder
yoho
young
zeliff
zimmer
aye
section
subsection
sec
act 
roll
yea
yes
nai
no
none
nay
mr
mrs
senator
gentleman
gentlemen
gentlewoman
gentlewomen
gentlelady
gentleladies
sir
committee
speaker
chairman
ask
yield
will
shall
can
say
let
adjourn
speak
etc
thank
absent
tell
per
part
now
month
today
con
pro
thereabout
thereafter
thereagainst
thereat
therebefore
therebeforn
thereby
therefor
therefore
therefrom
therein
thereinafter
thereof
thereon
thereto
theretofore
thereunder
thereunto
thereupon
therewith
therewithal
hereabout
hereafter
hereat
hereby
herein
hereinafter
hereinbefore
hereinto
hereof
hereon
hereto
heretofore
hereunto
hereunder
hereupon
herewith
whereabouts
whereas
whereafter
whereat
whereby
wherefore
wherefrom
wherein
whereinto
whereof
whereon
whereto
whereunder
whereupon
wherever
wherewith
wherewithal
bill
house
member
senate
amendment
section
subsection
committee
subcommittee
line
article
vote
insert
clerk
speaker
district
state
adjourn
monday 
tuesday
wednesday
thursday
friday
saturday
sunday
january
february
march
april
may
june
july
august
september
october
november
december
adjourn
board
general
legislature
legislation
parliament
amend
reject
appeal
appear
answer
appoint
ask
author
calendar
chair
chairman
colleague
commission
congress
court
file
motion
floor
leader
object
paragraph
unanimous
pending
revise
quorum
permission
secretary
resolution
pass
record
print
current
one
two
three
four
five
six
seven
eight
nine
ten
eleven
twelve
thirteen
fourteen
fifteen
sixteen
seventeen
eighteen
nineteen
twenty
thirty
fourty
fifty
sixty
seventy
eighty
ninety
hundred
hundreds
thousand
thousands
alabama
alaska
arizona
arkansas
california
colorado
connecticut
delaware
florida
georgia
hawaii
idaho
illinois
indiana
iowa
kansas
kentucky
louisiana
maine
maryland
massachussetts
michigan
minnesota
mississippi
missouri
montana
nebraska
nevada
hampshire
new
jersey
mexico
york
carolina
north
south
east
west
dakota
ohio
oklahoma
oregon
pennsylvania
island
rhode
tennessee
texas
utah
vermont
virginia
washington
wisconsin
wyoming
united

==> tables/all_sentiment.tex <==
\begin{tabular}{lr}
\hline
                           \textbf{Narrative} &  \textbf{Sentiment} \\
\hline
       people establish constitution &              0.9843 \\
              people promote welfare &              0.9843 \\
             founder endow men women &              0.9769 \\
            american take healthcare &              0.9643 \\
             veteran have healthcare &              0.9599 \\
            people establish justice &              0.9565 \\
                 kid have healthcare &              0.9564 \\
            family afford healthcare &              0.9531 \\
          small business provide job &              0.9531 \\
                   child have future &              0.9531 \\
. & . \\
. & . \\
. & . \\
             institute conduct study &             -0.9062 \\
          saddam hussein pose threat &             -0.9237 \\
                      people do harm &             -0.9300 \\
                  iraq pose jeopardy &             -0.9313 \\
               firefighter open fire &             -0.9325 \\
             terrorist kill american &             -0.9337 \\
                  child brought gift &             -0.9360 \\
                program provide help &             -0.9392 \\
               child have healthcare &             -0.9522 \\
       corrective action save family &             -0.9614 \\
\hline
\end{tabular}
